ABCTracker: an easy-to-use, cloud-based application for tracking multiple objects

Visual multi-object tracking has the potential to accelerate many forms of quantitative analyses, especially in research communities investigating the motion, behavior, or social interactions within groups of animals. Despite its potential for increasing analysis throughput, complications related to accessibility, adaptability, accuracy, or scalable application arise with existing tracking systems. Several iterations of prototyping and testing have led us to a multi-object tracking system -- ABCTracker -- that is: accessible in both system as well as technical knowledge requirements, easily adaptable to new videos, and capable of producing accurate tracking data through a mixture of automatic and semi-automatic tracking features.

==> Abstract.tex <==
Visual multi-object tracking has the potential to accelerate many forms of quantitative analyses, especially in research communities investigating the motion, behavior, or social interactions within groups of animals. Despite its potential for increasing analysis throughput, complications related to accessibility, adaptability, accuracy, or scalable application arise with existing tracking systems. Several iterations of prototyping and testing have led us to a multi-object tracking system – ABCTracker – that is: accessible in both system as well as technical knowledge requirements, easily adaptable to new videos, and capable of producing accurate tracking data through a mixture of automatic and semi-automatic tracking features. \newline \url{http://ABCTracker.org/}


==> Guided_Inference_Illustration.tex <==

    \begin{figure}[t!]
        \centering
            \includegraphics[width=\columnwidth]{Images/CorrectionInferenceExamples_ALT.pdf}
                \caption{[Caption here]}
            \label{GuidedInference}
    \end{figure}


==> Guided_Review_Example.tex <==

    \begin{figure}[ht!]
        \centering
            \includegraphics[width=\columnwidth]{Images/GuidedReviewExample_2.pdf}
                \caption{Illustration of a guided mode review. (Left) The video is zoomed (based on the size of the object) and a focus bubble is placed on the target. (Right) The user performs a click-n-drag interaction to define both the objects location and orientation (arrow length does not matter, only direction) and, once the interaction is complete, the system adjusts the zoom focus point and continues playback until the next key-frame is reached. Once all key-frames for the review have been annotated, the system (client) proceeds to the next review while inference is performed in parallel (on server).}
                \noteChange[inline]{(automatic video zoom based on target size -- prolly in figure caption)}
            \label{GuidedModeExample}
    \end{figure}


==> TrackingEvalTable.tex <==

    \begin{table*}[h]
        
        \caption{...}
        \noteImprove[inline]{Tracking run already - need to evaluate, but I'll have to correct the videos. They are not provided a "real" ground truth file, but rather something like the validation of crossings.}
        \label{Error-tracking-Evaluation}
            \begin{center}
                \begin{tabular}{ || c | c | c | c | c | c | c | c | c | c || }
                    \hline
                    Video     
                        & NumTargets 
                        & NumFrames 
                        & Frags   
                        & IDS 
                        & Hard IDS
                        & GT Coverage
                        & \% correct
                        & \% incorrect
                        & FAF  
                    \\ \hline \hline
                    
                    tadpole   
                        & ...
                        & ...
                        & ...
                        & ...
                        & ...
                        & ...
                        & ...
                        & ...
                        & ...    \\ \hline
                    cockroach   
                        & ...
                        & ...
                        & ...
                        & ...
                        & ...
                        & ...
                        & ...
                        & ...
                        & ...    \\ \hline
                    zebra-fish   
                        & ...
                        & ...
                        & ...
                        & ...
                        & ...
                        & ...
                        & ...
                        & ...
                        & ...    \\ \hline
                    etc..
                        & ...
                        & ...
                        & ...
                        & ...
                        & ...
                        & ...
                        & ...
                        & ...
                        & ...    \\ \hline
                    \hline
                \end{tabular}
        \end{center}
        
        
    \end{table*}

